Exploring Apache Incubator Project Trajectories with APEX

Open Source Software (OSS) is a major component of our digital infrastructure, yet more than 80% of such projects fail. Seeking less uncertainty, many OSS projects join established software communities, e.g., the Apache Software Foundation (ASF), with established rules and community support to guide projects toward sustainability. In their nascent stage, ASF projects are incubated in the ASF incubator (ASFI), which provides systematic mentorship toward long-term sustainability. Projects in ASFI eventually conclude their incubation by either graduating, if successful, or retiring, if not. Time-stamped traces of developer activities are publicly available from ASF, and can be used for monitoring project trajectories toward sustainability. Here we present a web app dashboard tool, APEX, that allows internal and external stakeholders to monitor and explore ASFI project sustainability trajectories, including social and technical networks.

==> MSR'22 Tool Demo Paper/extras.tex <==
\begin{itemize}
\item Email network data $\rightarrow$ Initial CSV file with developer names and receiver names $\rightarrow$ Final JSON format needed $\rightarrow$ \\ \lbrack sender\_name, receiver\_name, num\_emails between them\rbrack
\item Technical network data $\rightarrow$ Initial CSV file with developer names and file names $\rightarrow$ Final JSON format needed $\rightarrow$ \lbrack developer\_name, file\_name, num\_commits\rbrack

\item Email Metrics Data $\rightarrow$ Initial CSV file with developer names and receiver names $\rightarrow$ Final JSON format needed $\rightarrow$ \\ \lbrack num\_emails, num\_senders,email\_per\_developer \rbrack


\item Commit Metrics Data $\rightarrow$ Initial CSV file with developer names and file namess$\rightarrow$ Final JSON format needed $\rightarrow$ \lbrack num\_commits, num\_committers ,commit\_per\_developer \rbrack
\item About Projects data $\rightarrow$ JSON File containing $\rightarrow$ Project name, Sponsor, About, Mentors
\item Reports or Progress Data $\rightarrow$ Text file $\rightarrow$ containing the report or the progress report in a text format

\item Sustainability Forecast Data: The project sustainability forecast is a .json file containing key-value where the key is the project and the value is the monthly sustainability forecast.


==> extras.tex <==
\begin{itemize}
\item Email network data $\rightarrow$ Initial CSV file with developer names and receiver names $\rightarrow$ Final JSON format needed $\rightarrow$ \\ \lbrack sender\_name, receiver\_name, num\_emails between them\rbrack
\item Technical network data $\rightarrow$ Initial CSV file with developer names and file names $\rightarrow$ Final JSON format needed $\rightarrow$ \lbrack developer\_name, file\_name, num\_commits\rbrack

\item Email Metrics Data $\rightarrow$ Initial CSV file with developer names and receiver names $\rightarrow$ Final JSON format needed $\rightarrow$ \\ \lbrack num\_emails, num\_senders,email\_per\_developer \rbrack


\item Commit Metrics Data $\rightarrow$ Initial CSV file with developer names and file namess$\rightarrow$ Final JSON format needed $\rightarrow$ \lbrack num\_commits, num\_committers ,commit\_per\_developer \rbrack
\item About Projects data $\rightarrow$ JSON File containing $\rightarrow$ Project name, Sponsor, About, Mentors
\item Reports or Progress Data $\rightarrow$ Text file $\rightarrow$ containing the report or the progress report in a text format

\item Sustainability Forecast Data: The project sustainability forecast is a .json file containing key-value where the key is the project and the value is the monthly sustainability forecast.

